Non-Holonomic RRT & MPC: Path and Trajectory Planning for an Autonomous Cycle Rickshaw

This paper presents a novel hierarchical motion planning approach based on Rapidly-Exploring Random Trees (RRT) for global planning and Model Predictive Control (MPC) for local planning. The approach targets a three-wheeled cycle rickshaw (trishaw) used for autonomous urban transportation in shared spaces. Due to the nature of the vehicle, the algorithms had to be adapted in order to adhere to non-holonomic kinematic constraints using the Kinematic Single-Track Model. The vehicle is designed to offer transportation for people and goods in shared environments such as roads, sidewalks, bicycle lanes but also open spaces that are often occupied by other traffic participants. Therefore, the algorithm presented in this paper needs to anticipate and avoid dynamic obstacles, such as pedestrians or bicycles, but also be fast enough in order to work in real-time so that it can adapt to changes in the environment. Our approach uses an RRT variant for global planning that has been modified for single-track kinematics and improved by exploiting dead-end nodes. This allows us to compute global paths in unstructured environments very fast. In a second step, our MPC-based local planner makes use of the global path to compute the vehicle's trajectory while incorporating dynamic obstacles such as pedestrians and other road users. Our approach has shown to work both in simulation as well as first real-life tests and can be easily extended for more sophisticated behaviors.

==> sections/backup.tex <==

\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{\textwidth}
        \includegraphics[width=\textwidth]{NHRRT/nhrrt_2.png}
        \subcaption{Generating random point q\_rand and finding the nearest node q\_nearest inside the tree.}
        \label{fig:nhrrt1}
    \end{subfigure}
    \\
    \begin{subfigure}[t]{\textwidth}
        \includegraphics[width=\textwidth]{NHRRT/nhrrt_3.png}
        \subcaption{Using discretized steering angles, the nearest node is expanded into several children (marked as blue). The nearest child node is then selected.}
        \label{fig:nhrrt2}
    \end{subfigure}
    \\
    \caption{A visualization of the Non-holonomic RRT algorithm.}
    \label{fig:nhrrttree}
\end{figure*}


\begin{equation}
    \min_{\textbf{u}(t)}  \int_{t=t_s}^{t_s + T} \gamma(\textbf{x}(t), \textbf{u}(t)) \, dt + \Gamma_f(\textbf{x}(t_s + T))
    \label{eqn:bigmpc}
\end{equation}
\begin{alignat*}{2}
& \textrm{subject to:} \\
&    \textbf{x}(t_s) = \textbf{x}_s &
&    \textbf{\dot{x}}(t) = \textbf{f}(\textbf{x}(t), \textbf{u}(t)) \\
&    \textbf{x}(t_s + T) \in \mathbb{X}_f(t_s) \quad &
&    \textbf{x}(t) \in \mathbb{X}(t) \\
&    \textbf{u}(t) \in \mathbb{U}(\textbf{x}(t), t) \quad &
&    \textbf{\dot{u}}(t) \in \mathbb{U}_d 
\end{alignat*}

% \begin{wrapfigure}{l}{\linewidth}
%   \begin{center}
%     \subcaption{Generating random point q\_rand and finding the nearest node q\_nearest inside the tree.}
%     \label{fig:nhrrt2}
%   \end{center}  
%   \begin{center}
%     \includegraphics[width=\linewidth]{NHRRT/nhrrt_3.png}
%     \subcaption{Using discretized steering angles, the nearest node is expanded into several children (marked as blue). The nearest child node is then selected.}
%     \label{fig:nhrrt2}
%   \end{center}
%   \caption{A visualization of the Non-holonomic RRT algorithm.}
% \end{wrapfigure}

\begin{equation}
    \label{eqn:smallmpc}
    \min_{\textbf{u}}  \sum_{k=0}^{N-1} \gamma(\textbf{x}_k, \textbf{u}_k) \Delta t + \Gamma_f(\textbf{x}_N) \quad
\end{equation}
\begin{alignat*}{2}
& \textrm{subject to:} \\
&    \textbf{x}_0 = \textbf{x}_s &
&    \textbf{x}_{k+1} = \textbf{f}(\textbf{x}_k, \textbf{u}_k) \\
&    \textbf{x}_k \in \mathbb{X}(k \Delta t) \quad &
&    \textbf{u}_k \in \mathbb{U}(\textbf{x}_k, k \Delta t) \\
&    T = N \Delta t & 
&    k = 0, 1, 2, ..., N-1 
\end{alignat*}

In practical applications, the length does not need to be penalized as long as the planning horizon is smaller than the global lookahead distance. If that is the case, the planner will never be able to reach the target point $\mathbf{x}_{target}$ in a single iteration and will therefore always choose the path leading closest to it. For example, if the global lookahead distance is set to $\SI{10}{m}$, the planning horizon is set to $\SI{6}{s}$ and the maximum vehicle speed is $\SI{1}{m/s}$, the furthest the vehicle can plan into the future is $\SI{6}{m}$, which is less than the global lookahead distance, and therefore, the path length does not need to be penalized. 

Another highway driving scenario that focuses on collision avoidance is presented in \cite{7251458}. The authors employ time-varying safety constraints with model predictive control on a non-holonomic vehicle. The approach has been tested in simulation on three scenarios including lane shifting, stopping and overtaking. The controller was able to keep up with the demand and generate safe trajectories while avoiding collision.

Similarly, in \cite{7995716}, the authors also developed a path planning approach for highway driving using model predictive control. The approach focuses on lane change, lane keeping, ramp merging and intersection crossing scenarios. The authors also introduce potential field functions to achieve natural and comfortable maneuvers. 


In \cite{8289418}, the authors tackle the problem of lane change decision making and control via MPC. Having modeled the environment and predicted behaviour, a stochastic model predictive controller is employed to generate steering angle and linear velocity commands. The approach was tested in a simulation environment and in real life on a test vehicle, where the algorithm has proven to reliably handle complicated lane change scenarios with guaranteed safety. 



Unlike the local planner, which computes a trajectory, the global planner does not take into account dynamic obstacles such as cars or pedestrians. Therefore, the prerequisites for planning are very simple. In order to correctly function, the global planner only needs a map and the starting and goal positions.

In each iteration, the first set of values $\mathbf{u} = [v_0, \delta_0]^T$ is returned. 


The sum of times $ T = \sum_i \Delta t_i $ the planning horizon and represents how far the algorithm will plan into the future. Because the planner is called with a constant frequency of $f$ Hertz, the first command of the sequence $\mathbf{u}$ is applied for a total time of $ \Delta t_0 = 1 / f $. In order to simplify the problem, the duration $\Delta t$ can be set to a fixed value $ \Delta t_0 = \Delta t_1 = \Delta t_2 = ... = \Delta t_{n-1} = \Delta t $, dictated by the frequency $f$ of the planner, such that $ \Delta t = 1 / f$.

Another problem which arises is that due to the dynamic nature of the obstacles, the planner sometimes has trouble keeping up with the changing environment, causing the vehicle to come to an immediate stop (to avoid collisions with pedestrians) and request a re-planning of the global path. This can become problematic in crowds where numerous re-planning attempts would be made.

and has been tested on Segway RPMs, which were able to navigate at speeds of $ \SI{3.5}\;{m/s} $. The approach was also tested on the Sydney-Berkeley DARPA Grand Challenge vehicle for a combined total of hundreds of driving hours. 

Over the period of a few months, several tests have been conducted live on the vehicle, with the most important improvements and highlights being recorded and uploaded to YouTube. The recordings of the planner and vehicle in action can be found in continuation:

\begin{itemize}
    \item \url{https://youtu.be/Sm1tj7WEJLQ} - The purpose of this video is to highlight the vehicle's ability to follow a path provided by the global planner and reach the given goal region;
    \item \url{https://youtu.be/Rnf0l_RLoyo} - This video highlights the vehicle's ability to avoid pedestrians, where it successfully moved and avoided the cameraman and operator, even when jumping directly in front of the vehicle;
    \item \url{https://youtu.be/grg-59TbCVY} - This video represents the most recent test (as of the time of writing this paper), conducted on the 26.02.2021. The vehicle was able to drive autonomously for prolonged periods of time without leaving the designated driving area or crashing into obstacles. 
\end{itemize}

The purpose of the global planner is to compute a path from a starting pose $[x_0, y_0, \theta_0]$ to a goal pose $[x_n, y_n, \theta_n]$ on a given map without colliding into obstacles on the map. A global plan $\mathcal{X}$ as returned by the planner is therefore an array of individual states as presented in \autoref{eqn:globalpath}. Each state consists of two coordinates $(x,y)$ and a heading $\theta$. The first state  of the array, indexed by $0$, is the starting pose, whereas the last state, indexed by $n$ is the goal state. The size of the path is not predefined.

In the sampling phase, a point $q\_rand$ with $(x,y)$ is randomly generated inside the unoccupied area of the map. After that, the tree is searched and the state $q\_nearest$, which is closest to the randomly sampled point $q\_rand$, is selected. This is illustrated in the upper image of \autoref{fig:nhrrt}. In the extension phase, the selected state is expanded in the direction of the randomly sampled point. This process is repeated until one of the extended states is within the goal region defined on the map.


Another approach that solves motion planning for mobile robots based on MPC is presented in~\cite{5152240}. The authors suggest an approach for real-time sensor-based motion planning under kinodynamic constraints in dynamic environments. They use randomized sampling to construct a search tree in a similar fashion to RRT and then present improvements such as re-usage of trajectories. The approach also features the usage of waypoints as a guidance strategy.


\begin{figure*}[t]
    \centering
    \framebox[\textwidth]{\parbox{0.99\textwidth}{\includegraphics[width=0.99\textwidth]{figures/SystemArchitecture.pdf}}}
    % \includegraphics[width=0.99\textwidth]{figures/SystemArchitecture.pdf}
    \caption{A simplified system architecture highlighting our vehicle's key components for locomotion. \vspace{-3mm}}
    \label{fig:sys_arch}
\end{figure*}


\begin{algorithm}
\caption{Extend Children}
\label{alg:expansion}
\begin{algorithmic}[1]
\State $children = \{\}$
\State $range = max\_steering\_angle - min\_steering\_angle$
\For{$i \leq steering\_samples$}
\State $\delta \gets  min\_steering\_angle + (i / steering\_samples) \cdot range$
\State $child\_node \gets parent\_node$
\For{$j \leq step\_size$}
\State $child\_node.x \gets child\_node.x + v \cdot \cos(child\_node.\theta) \cdot T$
\State $child\_node.y \gets child\_node.y + v \cdot \sin(child\_node.\theta) \cdot T$
\State $child\_node.\theta \gets child\_node.\theta + v / L \cdot \tan(\delta) \cdot T$
\State $j \gets j +  integration\_step\_size$
\EndFor
\State $children.insert(child\_node)$
\State $i \gets i + 1$
\EndFor

\end{algorithmic}
\end{algorithm}
